OpenStereo: A Comprehensive Benchmark for Stereo Matching and Strong Baseline

Stereo matching aims to estimate the disparity between matching pixels in a stereo image pair, which is important to robotics, autonomous driving, and other computer vision tasks. Despite the development of numerous impressive methods in recent years, determining the most suitable architecture for practical application remains challenging. Addressing this gap, our paper introduces a comprehensive benchmark focusing on practical applicability rather than solely on individual models for optimized performance. Specifically, we develop a flexible and efficient stereo matching codebase, called OpenStereo. OpenStereo includes training and inference codes of more than 10 network models, making it, to our knowledge, the most complete stereo matching toolbox available. Based on OpenStereo, we conducted experiments and have achieved or surpassed the performance metrics reported in the original paper. Additionally, we conduct an exhaustive analysis and deconstruction of recent developments in stereo matching through comprehensive ablative experiments. These investigations inspired the creation of StereoBase, a strong baseline model. Our StereoBase ranks 1st on SceneFlow, KITTI 2015, 2012 (Reflective) among published methods and achieves the best performance across all metrics. In addition, StereoBase has strong cross-dataset generalization. Code is available at \url{https://github.com/XiandaGuo/OpenStereo}.

==> table_tex/Kitti15_leadboard.tex <==
\begin{table}
    \centering
    \vspace{-0.4cm}
    \caption{Quantitative evaluation on KITTI2015 leadboard.}
    % \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{l|c|c|c}
    \hline
    \multirow{2}{*}{\centering Method} &  \multicolumn{3}{c}{KITTI2015} \\
    % & \multicolumn{2}{c|}{KITTI2012(all)} &\multicolumn{2}{c}{KITTI2015(all)} \\ 
      \cline{2-4} 
      & D1-bg&D1-fg& D1-all \\
      % & 3px Error& epe(px) & 3px Error& epe(px)  \\
      \hline
     PSMNet~\cite{psmnet2018}&1.86 &4.62&2.32 \\ 
     PSMNet~\cite{psmnet2018}$^\dagger$& \textbf{1.80}&\textbf{4.58}&\textbf{2.26} \\ 
     \hline
     IGEV~\cite{xu2023iterative}& \textbf{1.38}&2.67&\textbf{1.59} \\
     IGEV~\cite{xu2023iterative}$^\dagger$&1.44 &\textbf{2.31}&\textbf{1.59} \\
    \hline
    \end{tabular}
    % }
\label{tab:kitti15_leadboard}
% \vspace{-0.8cm}
\end{table}

==> table_tex/SceneFlow.tex <==
\begin{table}[htbp]
    \centering
    % \vspace{-0.6cm}
    \caption{Quantitative evaluation on the SceneFlow~\cite{sceneflow} test. For each model, the specific category on the SceneFlow used is consistent with the original paper. Models marked with $^\dagger$ are OpenStereo implementations, others are from the original paper. Underline refers to evaluation in the non-occluded regions only~\cite{STTR}. Bold: Best}
    % \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{l|c|c|c}
    \hline
      \multirow{2}{*}{\centering Method} & \multicolumn{3}{c}{SceneFlow} \\ 
      % \cline{2-9} 
      & TrainSize & Categories & EPE(px) \\

      \hline 
       STTR~\cite{STTR} &$256\times512$& FinalPass& \underline{0.43} \\
       STTR~\cite{STTR}$^\dagger$ &$256\times 512$& FinalPass& \underline{0.40} \\

    
      % \hline 
       % RAFT-Stereo~\cite{raftstereo} &$256\times 512$& FinalPass& - \\
       % RAFT-Stereo~\cite{raftstereo}$^\dagger$ &$256\times 512$& FinalPass&1.18 \\
       
       \hline
       PSMNet~\cite{psmnet2018} &$256\times 512$& CleanPass &1.09 \\
       PSMNet~\cite{psmnet2018}$^\dagger$ &$256\times 512$& CleanPass&\bf{0.96} \\
       
       % \hline 
       % GANet~\cite{ganet2019} &$240\times 528$& CleanPass& 0.78 & -&- & -&- & -  \\
       % GANet~\cite{ganet2019}$^\dagger$ &$240\times 528$& CleanPass& \bf{0.65}& $240\times528$ &- &- &- & -  \\
            
       
       \hline 
       CFNet~\cite{cfnet2021} &$256\times 512$& FinalPass&1.04  \\
       CFNet~\cite{cfnet2021}$^\dagger$ &$256\times 512$& FinalPass&\bf{0.96}    \\
       
          
       % \hline 
       % DeepPruner~\cite{deeppruner2019} &$256\times 512$& CleanPass& 0.86\\
       % DeepPruner~\cite{deeppruner2019}$^\dagger$ &$256\times 512$& CleanPass& 0.86\\

       \hline 
       AANet~\cite{xu2020aanet} &$288\times 576$& CleanPass& 0.87 \\
       AANet~\cite{xu2020aanet}$^\dagger$ &$288\times 576$& CleanPass& \bf{0.80} \\ 
       
       \hline 
       Mobilestereo-2D~\cite{shamsafar2022mobilestereonet} &$256\times 512$& FinalPass& 1.14\\
       Mobilestereo-2D~\cite{shamsafar2022mobilestereonet}$^\dagger$ &$256\times 512$& FinalPass& \bf{1.10} \\ 
       Mobilestereo-3D~\cite{shamsafar2022mobilestereonet} &$256\times 512$& FinalPass& 0.80\\
       Mobilestereo-3D~\cite{shamsafar2022mobilestereonet}$^\dagger$ &$256\times 512$& FinalPass& \bf{0.79} \\ 

        \hline 
       GwcNet~\cite{gwcnet2019} &$256\times 512$& FinalPass& 0.76 \\
       GwcNet~\cite{gwcnet2019}$^\dagger$ &$256\times 512$& FinalPass& \bf{0.74}\\
       
       \hline 
       COEX~\cite{bangunharcana2021coex}&$288\times 576$& FinalPass&0.68 \\
       COEX~\cite{bangunharcana2021coex}$^\dagger$ &$288\times 576$& FinalPass&\bf{0.67} \\

       \hline 
       FADNet++~\cite{wang2021fadnet++} &$384\times 768$& CleanPass&0.76  \\
       FADNet++~\cite{wang2021fadnet++}$^\dagger$ & $384\times 768$& CleanPass& \bf{0.65}  \\
       
       \hline 
       CascadeStereo~\cite{gu2020cascade}&$256\times 512$& FinalPass& 0.72\\
       CascadeStereo~\cite{gu2020cascade}$^\dagger$ &$256\times 512$& FinalPass&\bf{0.67} \\
       
       % \hline 
       % ACVNet~\cite{acvnet} &$288\times 576$& FinalPass& 0.48\\
       % ACVNet~\cite{acvnet}$^\dagger$ &$288\times 576$& FinalPass&0.59 \\

       \hline 
       IGEV~\cite{xu2023iterative} &$320\times 736$& FinalPass& 0.47\\
       IGEV~\cite{xu2023iterative}$^\dagger$ &$320\times 736$& FinalPass&\bf{0.46} \\
    \hline
    \end{tabular}
% }
    \label{tab:sceneflow}
    % \vspace{-0.8cm}
\end{table}


==> table_tex/ablation_agg.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet3'
\begin{table}[htbp]
  \centering
  \caption{Ablation study results of cost volume on the Finalpass of SceneFlow test datasets~\cite{sceneflow}. Gwc represents group-wise correlation volume. Inter stands for Interlaced Volume. }
  \begin{threeparttable}
    \begin{tabular}{l|c|c}
    \hline
    Model & cost aggregation & \multicolumn{1}{l}{EPE} \\
    \hline
    \multirow{3}[0]{*}{Gwc8} & corr\_stem+hourglass & 0.7157 \\
          & corr\_feature\_att+hourglass & 0.7197 \\
          & hourglass & 0.7157 \\
    \hline
    \end{tabular}%
    
  % \vspace{3mm} % Adjust the 5mm to whatever space you desire
  %   \begin{tablenotes}[flushleft]
  %   \begin{minipage}{0.48\textwidth}
  %   \small
  %   \item \textit{Note:} Data augmentation combined random crop (320x760) with color augmentation and erasure transform, while scaling was also applied. Cost volume used group-wise correlation~\cite{gwcnet2019} with 8 channels. Context-upample~\cite{teed2020raft} strategies were applied for the final disparity regression.
  %   \end{minipage}
  %   \end{tablenotes}  
  \end{threeparttable}
  \label{tab:ablation_agg}%
\end{table}%


==> table_tex/compasion_other_methods.tex <==
\begin{table*}[htbp]
    \centering
    \vspace{-0.5cm}
    \caption{Quantitative evaluation on Scene Flow test set. Bold: Best.}
    \resizebox{0.98\textwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \hline
Method&PSMNet~\cite{psmnet2018}&MS3D~\cite{shamsafar2022mobilestereonet}&GwcNet~\cite{gwcnet2019}&COEX~\cite{bangunharcana2021coex}&FADNet++~\cite{wang2021fadnet++}&CStereo~\cite{gu2020cascade}&IGEV~\cite{xu2023iterative}&\textbf{StereoBase} \\
    \hline
    % Flops& 257.07G &154.38G&260.90G&13.45G&35.13G&303.29G&134.30G&559.81G&382.35G \\
    EPE(px)&1.09&0.80&0.76&0.68&0.76&0.72&0.46&\textbf{0.43} \\ 

    \hline
    \end{tabular}
    }
\label{tab:comparision_with_other}
\vspace{-1cm}
\end{table*}
